BioGen: Automated Biography Generation

A biography of a person is the detailed description of several life events including his education, work, relationships, and death. Wikipedia, the free web-based encyclopedia, consists of millions of manually curated biographies of eminent politicians, film and sports personalities, etc. However, manual curation efforts, even though efficient, suffers from significant delays. In this work, we propose an automatic biography generation framework BioGen. BioGen generates a short collection of biographical sentences clustered into multiple events of life. Evaluation results show that biographies generated by BioGen are significantly closer to manually written biographies in Wikipedia. A working model of this framework is available at nlpbiogen.herokuapp.com/home/.

==> bioGenProcess.tex <==
\section{Methodology}
A biography can be defined as an account of the series of facts and events that
make up a person's life. Different types of biographical facts include aspects related to personal characteristics like date and place of birth, date and place of death, education, career, occupation, affiliation and relationships. 
Understanding the information that should be present in a biography, in this section we describe a process for an automatic generation of a biography given some set of documents. The biography generation process can be described in three major steps (A) \emph{Identifying Biographical Sentences}, (B)  \emph{Classifying Biographical Sentences}, and (C) \emph{Summarization}. In the sections below (\ref{sec:2_class}, \ref{sec:6_class}, and \ref{sec:summarizer}), we describe each of the steps in detail. Along with the biographical  information, a Wikipedia page of a person also consists of a consistently-formatted table on the top right hand size of the page. This table or box is known as \emph{infobox}, and it contains some important facts related to the person. For completeness, we describe a process (in section \ref{sec:infobox}) to generate a table or \emph{infobox} similar to the one present on the Wikipedia page.
%We developed the approach considering the above classes into consideration.
\subsection{Identifying Biographical Sentences}
\label{sec:2_class}
Given a document that describes an event or some news related to a person, note that, not all the sentences from that document appear in a biography. So, in order to generate a biography, first there is a need to identify whether a particular sentence would really appear in the biography or not. The facts that appear in a biography are mostly expressed in the form of complete sentences.
Given a sentence, its very likely that a human can identify whether that sentence would appear in person's biography or not. However, this task might not be that easy for a machine. A machine should first learn to identify the difference between a biographical and non-biographical sentences. To make this task easier for the machine, we train a Machine Learning model that can differentiate between biographical and non-biographical sentences. The datasets that we use to train the  classifier are (1) \texttt{TREC} and (2) \texttt{WikiBio}. 
Details about these Datasets are given in section 5.1

Before feeding the data to the classifier, we first do some basic preprocessing to clean the data. Then, each document is segmented into sentences and each sentence is vectorized using a \texttt{TF-IDF} vectorizer. Now, this vector acts as a data point for the classifier, and the class label for each vector is either 1 or 0 depending on whether it is a \texttt{biographical} sentence or not. We assume that, all the sentences that are present in the \texttt{WikiBio} dataset (described in section \ref{sec:datasets}) are are biographical sentences (class label 1) and the sentences that are present in the \texttt{TREC} dataset (described in section \ref{sec:datasets}) are \texttt{non-biographical} sentences (class label 0).
%This will encode sentences into vectors. Then we classify into one of two base categories, namely biographical and non-biographical. 
We feed these data points to three different binary classification methods such as Logistic Regression, Decision Trees and Naive Bayes. For this dataset, the Logistic Regression based model gives highest  %({\color{red}{train or test??}})%
accuracy (around 96\%) on test data and thus we use it for the steps further.
%non-biographical sentences using Logistic Regression The accuracy of two class classifier is 96\% which is quite promising. 

Before going to the next step, we filter out some biographical sentences which does not contain any Named Entity Tags like \emph{PERSON}, \emph{PLACE} or \emph{ORGANIZATION}, as these sentences might not add much value and meaningful information to the biography.
As our main aim to generate a biography as similar to that of the Wikipedia page, where there are number of different sections present, our next step is to identify for each biographical sentence which is the appropriate section. 
\subsection{Classifying Biographical Sentences}
\label{sec:6_class}
Here, we employ a new classifier to classify a sentence to a particular section. The first challenge here is to get such a dataset where each sentence is labeled to a particular section. For this we use the \texttt{BigWikiBio} dataset (described in section \ref{sec:datasets}). We annotate/label each sentence in the dataset by its first/second heading as per the Wikipedia page. For now, we restrict ourselves to six broad and important classes (sections) namely \emph{Education, Career, Life, Awards, Special Notes and Death}. Each of these broad categories can be thought of as containing sentences from various sections. For eg. the sentences from the sections \emph{College, High School, Early life and education, Education, etc.} are tagged into the \emph{Education} class. Similarly, the other broad categories contain sentences from some similar classes.
%as follows:\par
% \begin{enumerate}
% {\textbf{Education:}} College, High School, Early life and education, Education, etc. \par
% {\textbf{Career:}} Politics, Music career, Career, Works, Publications, Research, etc. \par
% {\textbf{Life:}} Early life, Family, Marriage, History, Personal life, etc.\par
% {\textbf{Honours/Awards:}} Honors, Awards, Recognition, Championships, Achievements, Accomplishments, etc.\par
% {\textbf{Special Notes:}} Notes, Legacy, Personal, Gallery, Influences, Other, Controversies, etc.\par
% {\textbf{Death:}} Death, Death and Legacy, Later life and Death, etc.\par
% \end{enumerate}
We believe that this can be easily extended to more classes/sections. For this multi-class classification task we train a Logistic Regression based model.
The generated biography is thus automatically divided into sections pertaining to various different aspects in the life of a person.

After this step, we have the sentences that are biographical sentences and are also divided into various section headings. However, there can be some duplicate sentences or information present. Also, the biography must be as succinct as possible. Thus, our next step is the summarization step which helps in generating a compact and condensed biography.


%We used Logistic Regression and trained a classifier on our dataset.
% Highest occurring headings were chosen to constitute the six classes. The grouping was done as following:
% The sentences which are categorized as \texttt{biographical} are then further classified into 6 major classes consisting of \emph{Education, Career, Life, Awards, Special Notes and Death} 
% For training these 6 classes we created our own dataset. We scraped the data of six million Wikipedia biographies and annotated each sentence by its first/second headings, as available in the Wikipedia biography. 
% For training the 6 classes We scraped the data of six million wikipedia biographies and annotated each sentence by its first/second headings, as available in the Wikipedia biography we took Top 6 classes based on Heading frequencies and then we trained our classifier on these 6 classes. We assigned all the different types of headings matching with a class title to one of the classes. The grouping was done as following
% Each sentence in the test set falls into any one of the above classes. The generated biography is thus automatically divided into sections pertaining to various different aspects in the life of a person. 

\subsection{Summarization}
\label{sec:summarizer}
To get a concise biography, we apply {Text Rank based summarization \cite{mihalcea2004textrank}} on each of the six sections or classes using the  Gensim Summarizer \cite{rehurek_lrec}.
% Within the produced text, we still need a mechanism to generate only as long a biography as required by the user.  To achieve this, we use Text Rank based summarisation individually on each of the six classes. We use Gensim Summarizer for this purpose. 
This also imparts flexibility in terms of the length of the generated biography as the number of lines required in the output can be specified. 
The summarizer also helps in taking only the most important ideas and relevant information from the biography.

\iffalse
\begin{figure}[!tbh]
    \centering
    \includegraphics[width=0.8\hsize]{ApproachNLP.png}
    \caption{Overview of Approach}
    \label{fig:approach}
\vspace{-0.3cm}
\end{figure}
\fi

\subsection{Generating Infobox}
\label{sec:infobox}
Infobox is a well formatted table which gives a short and concise description of some important facts related to the person. The following are the facts/rows which we present in the Infobox of a person:

\textbf{Name:} This is same as that of the input query.
    
\textbf{Date of Birth \& Date of Death:} To extract these information from the text, we used regular expressions to extract the date and depending on the context (words such as `born on', or `birth') present nearby the date, the extracted date is associated with the events like day of birth or the day of death. 
%We checked for some specific words which are generally associated with sentences in which Date of Birth is generally present like `born', `birth', etc. and then extracted the date in that particular sentence.
% First we used POS Tagging t Used POS tagging and  Information Extraction from the sentences which contains Date and some information on Death.

\textbf{Place of birth:} The methodology used here is similar to that used in the extraction of \emph{Date of Birth}. Here to identify the exact place we used \emph{POS} tagging and \emph{Named Entity Recognition} from the Stanford NLTK Library {\cite{Bird:2009:NLP:1717171}}.
%\item \textbf{Date of Death:} Used POS tagging and  Information Extraction from the sentences which contains Dates and some information on Death

\textbf{Awards:} To extract this information from the sentences we checked for whether a sentence mentions any award name or not. If so, we just extract that award name and associate the award with the person for whom the biography is to be generated. In order to get the list of all the awards we used the information present at the \emph{Wikipedia List of Awards page} \footnote{https://en.wikipedia.org/wiki/List\_of\_awards}.

\textbf{Education \& Career:} To get the information about persons education and career we followed the approach as similar to the one used for the extraction of \emph{Awards}. We used the information present at official government sites like \texttt{data.gov.in} and \texttt{usa.gov} to get the education related information. And career related information was obtained from the Wikipedia page that mentions the \emph{list of Occupations} \footnote{https://en.wikipedia.org/wiki/Lists\_of\_occupations}.
% \end{itemize}

Generally, a Wikipedia page of a person consists of an image of a person as well. Even for the biographies generated as per our generation process, we extract an image of the person by doing a Google search query. This part is again for completeness of the generated biography.

==> intro.tex <==

 
\iffalse{}
As the Web technology continues to thrive, a large number of documents 
%containing biographical information 
are continuously generated and published online. Online newspapers, for instance, publish articles describing important facts or events related to the life of well-known individuals. 
However, all these facts or information mentioned in these published documents does not really become a part of biography of a person. But, these Web documents often contain both meaningful biographical facts, as well as additional contents irrelevant to describe the person (e.g., detailed accounts of the person actions). In order to generate a biography one needs to filter the content from these documents.      Although humans mostly manage to filter the
desired information, manual inspection does not scale to very large document collections. For example, a page on Wikipedia is generated by a contribution by number of authors which might have referred distinct
 documents. However, we believe that, if relevant biographical information in human generated
texts can be extracted automatically, then this information can be used in the production of structured biographical databases, capable of supporting many interesting studies in Humanities and related areas. With this as the motivation,  in this paper, we address the task of automatically extracting biographical facts from textual documents published on the Web. We propose to segment documents into sequences of sentences, afterwards classifying each sentence as describing either a specific type of biographical
fact, or some other case not related to biographical data. For classifying the sentences, we experimented with classification models based on the formalist of Naive Bayes, Logistic Regression and Conditional Random Fields using various sets of features for
describing the sentences. Experimental results attest for the adequacy of the proposed approaches, showing an F1 score of approximately 84\% in
the 2-class classification problem, 65\% for 7-class classification problem and 59\% for the 19-class classification problem.
In this paper we present automatic biography generation using extractive summarization. We trained our model so that it can select important sentences from the input documents. Generative models are highly complex and most of the summarizers often use extractive model for summarization.

Section 2 describes related literature.  Section 3 describes our problem statement. Section 4 describes the components of our system in more detail. Section 5 describes our experiments along with dataset Section 6 draws the final conclusion of our work.
\fi

==> probStatement.tex <==
\section {Problem statement}
In this project, we have worked on the problem of automatically generating a biography of a person, given some input documents (news articles, tweets, books) related to that person. We present an automatic approach using extractive summarisation techniques to generate a concise, multi sectioned biography of the person. An INFOBOX that highlights details about that person such as Date of Birth, Date of Death, Educational Qualification, etc is also generated by our system. Wikipedia is the best source for biographies as it is written manually. Our model also tries to generate biographies in a much more similar manner. Similar to Wikipedia's biography our model also separated information into various classes such as Education, Career, Honours and Awards. When given a set of documents news articles, books, tweets etc. our model first classifies those into two classes viz. biographical; and non biographical. This is done by a classifier. We trained our classifier by taking two data- sets viz. TREC \cite{lebret2016neural}
 and Wikipedia \cite{Amini:2009} for biographical and non-biographical sentences respectively. An important assumption taken is that we consider all the sentences taken from news articles as non biographical and those taken from Wikipedia as biographical.

==> rw.tex <==
\section{Related Work}
Majority of past literature focuses on Machine Learning techniques for information extraction. Zhou et al.~\cite{zhou2005multi} trained biographical and non-biographical sentence classifiers to select sentences. They used Naive Bayes based model with \texttt{n-gram} features to classify sentences into ten classes such as bio, fame factor, personality, etc.
%In contrast the framework that we propose does not require any manual effort for extracting features. 
Biadsy et al.~\cite{biadsy2008unsupervised} proposed  summarization techniques to extract important information from multiple sentences. This system uses a binary classifier for classifying sentences as biographical and non biographical. 
Liu et al.~\cite{liu2018generating} also use multi-document summarization. For identifying salient information, the paragraphs are ranked and ordered using various extractive summarization techniques. Filatova et al.~\cite{Filatova:2005} presented SVM-based techniques for identifying occupation related important events for generating biography. The work by Barzilay et al.~\cite{Barzilay:2001} focus on sentence ordering techniques in multi-document summarization.
One of the recent works in generating sentences is by Lebret et al.~\cite{lebret2016neural}. They use \emph{concept to text generation} approach to generate sentences using the fact tables present in Wikipedia. 

%The authors propose a Neural Language based model that exploits the structure in the facts data to generate text. Given the limited information used for training the model (i.e. only tables), the system is proposed to generate only the first sentence on Wikipedia page accurately. 

In contrast to the above mentioned works, we propose an automated framework that is build upon some simple classification models and information extraction techniques to generate a page as similar to that of Wikipedia. Also, the features required for the classification models are easy to extract and does not require manual effort. Along with the biography generation task, we also propose a method to generate \emph{Infobox} which is a consistently-formatted table mentioning some important facts and events related to a person. 
%Our system provides flexibility in choosing the length of the biography to be generated.
%In contrast, we are first classifying the sentences whether they are biographical or not using 2-class classifier and POS Tagging and then arranging the data into 6 classes using 6 class classifier trained on wikipedia data and creating the infobox of the person.Also, ours is an automated model.


